ViVid-1-to-3: Novel View Synthesis with Video Diffusion Models

Generating novel views of an object from a single image is a challenging task. It requires an understanding of the underlying 3D structure of the object from an image and rendering high-quality, spatially consistent new views. While recent methods for view synthesis based on diffusion have shown great progress, achieving consistency among various view estimates and at the same time abiding by the desired camera pose remains a critical problem yet to be solved. In this work, we demonstrate a strikingly simple method, where we utilize a pre-trained video diffusion model to solve this problem. Our key idea is that synthesizing a novel view could be reformulated as synthesizing a video of a camera going around the object of interest -- a scanning video -- which then allows us to leverage the powerful priors that a video diffusion model would have learned. Thus, to perform novel-view synthesis, we create a smooth camera trajectory to the target view that we wish to render, and denoise using both a view-conditioned diffusion model and a video diffusion model. By doing so, we obtain a highly consistent novel view synthesis, outperforming the state of the art.

==> figs/deg_vs_psnr/item.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/deg_vs_psnr/psnr.png}
    \caption{\TODO{deg\_vs\_psnr}}
    \label{fig:deg_vs_psnr}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> sec/3_method_OLD.tex <==
\input{figs/overview/item}

\section{Method}
\label{sec:method}

\ky{%
The key idea behind our method is strikingly simple, video diffusion models can be used as a strong prior conjunction with novel-view diffusion models for immediate improvement, \emph{without} any training of fine-tuning.
Instead of directly generating a novel view, we propose to generate a camera trajectory towards the camera view that we wish to render.
As illustrated in \cref{fig:overview}, while the novel-view diffusion model alone creates errors along the camera path, and is not consistent when it comes to the actual pose of the object that is rendered, with the help of a video diffusion model, which globally smooths out the individual frame outcomes to form a smooth, realistic video.
This results in both renderings that abides by the requested novel pose, as well as the contents being consistent with the input view.
}%

\ky{%
To explain our method, we first provide a brief overview diffusion models to introduce the notations that we will use (\cref{sec:prelim}).
We then detail our method (\cref{sec:main_method}) and discuss important implementation details (\cref{sec:impl}).
}%


% To foster consistency in novel view synthesis, we leverage the video diffusion models \cite{} that have shown promising results for generating smooth camera trajectories. 
% Our approach combines the diffusion models that generate novel views of an image conditioned on the camera pose \cite{} with the motion information in the video diffusion models yielding coherent continuous views of the image.
% In the following, we discuss diffusion models for novel view synthesis and video diffusion models which form the foundations of our approach.


\subsection{Preliminaries: Diffusion models}
\label{sec:prelim}

% Diffusion models typically consist of two processes, i.e., a forward process $q$ which gradually injects noise to data ${x}$ consecutively over $T$ steps to transit the original data distribution to Gaussian distribution, and a reverse process $p$ that includes denoising steps to reconstruct the data structure from a noisy image, where the denoiser computes the marginal distribution of an intermediate noisy image at timestep $t$ to predict a less noisy variable at timestep $t-1$. It is formulated as,
% \begin{align} \label{eq:diffusion_forward_backward}
% q\left(\mathbf{x}_t \mid \mathbf{x}_{t-1}\right)&=\mathcal{N}\left(\mathbf{x}_t ; \sqrt{1-\beta_t} \mathbf{x}_{t-1}, \beta_t \mathbf{I}\right), \\
% p_{\theta}\left(\mathbf{x}_{t-1} \mid \mathbf{x}_{t}\right)&= \mathcal{N}\left(\mathbf{x}_{t-1} ; \mu_\theta\left(\mathbf{x}_t, t\right), \sigma_t^2 \mathbf{I}\right).
% \end{align}
\paragraph{Diffusion models.} 
Latent Diffusion Models (LDMs) transform an input image $\mathbf{x}$ to noise by gradually adding Gaussian noise over $T$ steps of the forward diffusion process \cite{rombach2022high}. 
The forward and the reverse processes are applied in the latent space of a pre-trained autoencoder ~\cite{van2017neural, esser2021taming}. 
The objective of LDM is given by, 
\begin{equation} \label{eq:SD objective}
   \min \mathbb{E}_{\mathcal{E}\left(\mathbf{x}\right), \epsilon, t}\left[\left\|\epsilon-\epsilon_\theta\left(\mathbf{z}_{t}, t, y\right)\right\|_2^2\right],
\end{equation}
where $\mathcal{E}$, $\mathbf{z}_{t}$, and $y$ denote the pre-trained encoder, latent codes at timestep $t$ and conditioning prompt, respectively. 

% View-conditioned diffusion models~\cite{liu2023zero1to3,shi2023mvdream} that conducts novel view synthesis of objects take an single-view image and camera parameters as additional inputs.
% The embedding of camera transformation guides the diffusion process to generate a desired target view

\paragraph{Diffusion models for novel view synthesis.}
Given a single RGB image $\mathbf{x}$, the goal of novel view synthesis is to generate an image of the same object from a different camera viewpoint.
For the target camera $\mathbf{c}=[R\mid T]$, the relative camera rotation $R \in \mathbb{R}^{3 \times 3}$ and the translation of the desired
viewpoint $T \in \mathbb{R}^3$, the new image $\mathbf{x}_{c}$ is given by a transformation $f(\mathbf{x},R,T)$.
\TODO{R,t introduced but never used.}
In case of view-conditioned diffusion models~\cite{liu2023zero1to3,shi2023mvdream}, an embedding $\phi(\mathbf{x},\mathbf{c})$ encoding the camera extrinsics $R,T$ along with the input image $\mathbf{x}$ is provided as conditional information $y$ in Eq.~\ref{eq:SD objective} for view-conditioned image-to-image translation task.
Specifically, the embedding of the camera transformation with an input image guides the diffusion process parameterized by $\theta_{view}$ as:
\begin{equation} \label{eq:zero1to3 objective}
   \min \mathbb{E}_{\mathcal{E}\left(\mathbf{x}\right),\epsilon, t}\left[\left\|\epsilon-\epsilon_{\theta_{view}}\left(\mathbf{z}_{t}, t, \phi(\mathbf{x},\mathbf{c})\right)\right\|_2^2\right].
\end{equation}
Target images with desired views can thus be generated by conditioning on different camera extrinsic parameters.
%$\mathcal{F}_{\text{vc}}(\cdot)$ to generate a desired target view image $\hat{\mathbf{x}}$ , i.e., 
%\begin{equation}
%\hat{\mathbf{x}}  = \mathcal{F}_{\text{vc}}(\mathbf{x}, \mathbf{c}) 
%\end{equation}


\paragraph{Video diffusion models.} Video diffusion models aim to generate plausible and sequential video frames by guiding the diffusion process with an input prompt. Among them, latent video diffusion models~\cite{} have focused on improving inter-frame consistency in the latent space of pre-trained LDMs to harness the power of large-scale models. Therefore, the training objective of text-to-video diffusion parameterized by $\theta_{vid}$ can be represented as an extension of \cref{eq:SD objective} over the temporal dimension as, 
\begin{equation} \label{eq:videodiff}
   \min \mathbb{E}_{\mathcal{E}\left(\mathbf{x}_{0}^{(1:L)}\right), y, \epsilon, t}\left[\left\|\epsilon-\epsilon_{\theta_{vid}}\left(\mathbf{z}_{t}^{(1:L)}, t, y\right)\right\|_2^2\right],
\end{equation}
% to learn joint distribtuion of frames.
where $\mathbf{x}_{0}^{(1:L)}$ and $\mathbf{z}_{t}^{(1:L)}$ denote $L$ frames of input video and noisy latent codes at timestep $t$, respectively. Here, the objective in Eq.~\ref{eq:videodiff} encourages the model to learn joint distribution of the temporal frames. 


%\JG{TODO: check equations again (notations, bold}

%\TODO{some math notations and quick equations that we will use to write down our own model. Introduce zero123 and zeroscope models as black box here}



\subsection{Diffusion for consistent novel-view synthesis}
\label{sec:main_method}

View-conditioned diffusion models as formalized in \cref{eq:zero1to3 objective} are limited when constructing multiple views with consistency.
Consider a view-conditioned diffusion model parameterized by $\theta_\text{view}$ that is used to generate a set of multi-view images $\image^{1:N}=\{\image^1,...,\image^N\}$ according to a given camera trajectory
$\mathbf{c}^{1:N}=\{\mathbf{c}^1,\mathbf{c}^2,...,\mathbf{c}^N\}$ from a single image $\image^0$ in camera pose $\mathbf{c}^0$.  
Since the frames corresponding to different poses are processed independently of each other, the features of objects in images may be incoherent due to the stochastic diffusion process for each view \ie, 
\begin{equation}
    % p_\theta\left(\image_{0: T}^{(1: N)}\right)=
    % p\left(\mathbf{x}_T^{(1: N)}\right) \prod_{t=1}^T 
    p_{\theta_\text{view}}\left(\image_{t-1}^{1: N} \mid \image_t^{1: N},\mathbf{C}^{1:N} \right) = \prod_{n=1}^N p_{\theta_\text{view}}\left(\image_{t-1}^{n} \mid \image_t^{n},\mathbf{C}^n \right),
\end{equation}
where $\mathbf{C}^n=\phi(\image^{0}, \mathbf{c}^n)$ denotes an encoded vector of relative pose between the $n$-th segment of the camera trajectory $\mathbf{c}^n$ and  $\mathbf{c}^0$ along with the input $\image^0$.

To address the inconsistency in the view synthesis, several methods \cite{} have tried to model joint distribution for pre-defined fixed views, or exploited score distillation to NeRF \cite{}.
These approaches, however, require additional computational overhead for fine-tuning or optimization
or are capable of synthesizing only pre-defined views due to the restricted probability space.
%Moreover, these methods can synthesize only pre-defined views \SM{add why? Are they conditioned on specific poses}.
In this work, instead, we propose a zero-shot-based approach to achieve multi-view consistency without re-training or score distillation.  

\paragraph{Video diffusion as consistency prior.}
Video diffusion models encode smooth motion or camera trajectories with sequential frame generation (\cf~\cref{eq:videodiff}).
We leverage this motion prior to encourage consistency in multi-view synthesis with diffusion models.
To this end, we combine the strengths of the view synthesizing diffusion model~\cite{liu2023zero1to3} to guide generation according to each camera and that of video diffusion models in ensuring consistent transitions across frames of video.
% Given a reference image $\mathbf{I}^0$, we start generate $N$ views $\mathbf{I}^{1:N}$ of the image conditioned on the relative camera poses $c^{1:N}$ using view-conditioned diffusion model parameterized by ${\theta}_{view}$. }
Given a reference image $\mathbf{I}^0$, we start the reverse (denoising) process of video diffusion with $L$ noisy frames. 
Here, each camera pose yields a single view of the image.
The noise estimates at timestep $t$ from the view-conditioned model for the camera trajectory $\mathbf{c}^{1:L}$ are calculated independently for each frame, i.e., $\epsilon_{\theta_\text{view}}(\mathbf{z}_t^{1:L},t,\mathbf{C}^{1:L})=\{\epsilon_{\theta_\text{view}}(\mathbf{z}_t^{n},t,\mathbf{C}^{n})\}_{n=1}^{L}$. 
After that, we exploit a pre-trained text-to-video diffusion model~\cite{} parameterized by $\theta_\text{vid}$ to estimate the noise component $\epsilon_{\theta_\text{vid}}(\mathbf{z}_t^{1:L},t,y)$.
The video diffusion guides the alignment of these stochastic diffusion processes to improve inter-frame consistency.   
Here, we use an empty prompt as condition ($y=\O$) to faithfully inject view-dependent conditioning information from $\epsilon_{\theta_\text{view}}$. Intuitively, our strategy can be interpreted as formulating a multi-view synthesis problem into a video generation task by leveraging video diffusion as a universal consistency prior in a non-trivial fashion.

Our straightforward approach surprisingly improves the multi-view consistency by combining two pre-trained diffusion models, thus it brings us three noteworthy advantages: First, we do away with the need for score distillations~\cite{} or re-training in diffusion-based novel view generation. 
Secondly, our framework is capable of synthesizing arbitrary views unlike recent methods~\cite{} that only allow pre-defined several views.  
Finally, it offers flexibility in the choice of camera trajectory and number of cameras (frames).
%This noise estimate can be interpreted as points on the smooth camera trajectory of the video diffusion model. 

% We input the sequence of the generated frames $\mathbf{I}^{1:L}$ to a pre-trained video diffusion model parameterized by $\theta_{video}$ to estimate the noise component $\epsilon_{\theta_{video}}(\mathbf{z}_t^{1:L},t,y)$ where we use an empty prompt as condition. 
% With the two noise estimates at hand, we guide the video generative model to produce consistent views by injecting the noise components from the video diffusion model (see implementation details) into the view-conditioned diffusion model at a subset of timesteps $t' \in \{1,\ldots, T\}$ during inference.


%Given the starting reference view, and provide the camera trajectory not in terms of absolute value but relative value from reference view. Then we guide zero123 to generate target view, and then use video }

%\ky{%An overview of our method is provided in \autoref{fig:overview}.As shown, we use two different types of diffusion models, namely, one that generates novel views conditioned on the \JG{frontal $\rightarrow$ reference} image and the desired camera pose, and another that generates videos. We treat the novel view \JG{generation$\rightarrow$synthesis} problem as a generation problem, and basically ask the video diffusion model to generate a video that starts from the frontal image \jg{$\image^0$}\JG{changed $\image_0\rightarrow\image^0$ to avoid overlap with the diffusion step}, and follows a smooth camera trajectory to the desire view of the image \jg{$\image^V$}.To do so since the video diffusion models are not trained specifically to generate a certain camera trajectory, we basically rely on the novel view generation diffusion models to do this.}%

%\jg{
%In our framework, the camera trajectory consists of a set of $L$ camera poses $\mathbf{c}^{1:L}$ and also the video diffusion has the same number of frames as the number of cameras. Each frame is guided independently by the novel view diffusion for each camera. Here, the video diffusion process }


% \TODO{main method}
% \JG{TODO: Equations}
% \subsection{Handholding diffusion from drifting}
% \textbf{}
% \ky{%
% While \autoref{sec:main_method} provide basis on how the two diffusion models can be combined for consistent novel view synthesis, or attempts led to over-smoothed results due to diffusion models drifting.
% Thus, in order to prevent this, we propose to use regularization terms in the form of classifier guidance~\cite{}.
% Specifically, \TODO{}
% }%

\subsection{Implementation details}
\label{sec:impl}

\paragraph{Scheduling the noise weights}
\TODO{how much of each diffusion model}

\paragraph{Choice of Diffusion Models}

\paragraph{Hyperparmeter setup}
\TODO{Erqun was tuning these}


==> tbl/quantitative_flow.tex <==
\begin{table}
    \centering
    \begin{tabular}{c|c}
    \toprule
         &  \\
    \midrule
         & \\
    \bottomrule
    \end{tabular}
    \caption{{\bf Pose metrics -- }
    \TODO{caption}
    }
    \label{tab:quantitative_flow}
\end{table}
